Circular formation control of fixed-wing UAVs with constant speeds

In this paper we propose an algorithm for stabilizing circular formations of fixed-wing UAVs with constant speeds. The algorithm is based on the idea of tracking circles with different radii in order to control the inter-vehicle phases with respect to a target circumference. We prove that the desired equilibrium is exponentially stable and thanks to the guidance vector field that guides the vehicles, the algorithm can be extended to other closed trajectories. One of the main advantages of this approach is that the algorithm guarantees the confinement of the team in a specific area, even when communications or sensing among vehicles are lost. We show the effectiveness of the algorithm with an actual formation flight of three aircraft. The algorithm is ready to use for the general public in the open-source Paparazzi autopilot.

==> Makefile <==
all: iros2017_uav.pdf

clean:
	$(RM) *~ *.pdf *.dvi *.log *.aux *.bbl *.blg *.toc *.lol *.loa *.lox \
		*.lot *.out *.lg *.tmp *.xref *.lof .*.swp

iros2017_uav.pdf: iros2017_uav.tex
	pdflatex iros2017_uav
	bibtex iros2017_uav
	pdflatex iros2017_uav
	pdflatex iros2017_uav

